Strong local nondeterminism for stochastic time-fractional slow and fast diffusion equations

We study a class of stochastic time-fractional equations on $\mathbb{R}^d$ driven by a centered Gaussian noise, involving a Caputo time derivative of order $\beta>0$, a fractional (power) Laplacian of order $\alpha>0$, and a Riemann-Liouville time integral of order $\gamma\ge0$ acting on the noise. The noise is fractional in time (index $H$) and Riesz-type in space (index $\ell$). We derive sharp Dalang-type necessary and sufficient conditions for the existence of a random field solution across almost full parameter range $(\alpha,\beta,\gamma;H,\ell)$. Under the Dalang-type conditions, we prove sharp variance bounds for temporal and spatial increments, as well as strong local nondeterminism in time in several regimes (two-sided version for $\beta=1$ and for parts of the case $\beta=2$; one-sided version for $0<\beta<2$) and strong local nondeterminism in space for the whole range of parameters. As applications, we derive exact uniform and local moduli of continuity, Chung-type laws of the iterated logarithm, and quantitative bounds on small ball probabilities. Along the way, we obtain sharp asymptotics for the fundamental solution kernels at $0$ and $\infty$, which may be of independent interest.

==> preamble.tex <==
\usepackage[table]{xcolor}
\usepackage{amsmath, amsthm, amsfonts, amssymb, enumerate, xfrac, tikz, comment, pgfplots, mathtools}
\usepackage[most]{tcolorbox}
\usepackage{makeidx}
\makeindex
\usepgfplotslibrary{external}
\pgfplotsset{compat=1.18}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usetikzlibrary{shapes.geometric, positioning, matrix, decorations.pathreplacing, shadings, arrows}
\excludecomment{codes}
% \usepackage{showkeys}
% \usepackage{showlabels}
\usepackage{empheq}
\usepackage{multicol}

% -------------------------------------------------
% Set up the page margins.
% -------------------------------------------------
\usepackage[text={6.5in,9.0in},centering]{geometry}
% \setlength{\topmargin}{-0.25in}


% -------------------------------------------------
% Load Packages here
% -------------------------------------------------
\usepackage{graphicx,url}
\RequirePackage[OT1]{fontenc}
\usepackage{datetime}
\usepackage{tikz-3dplot}
\usepackage{subcaption}
\usepackage[normalem]{ulem} % either use this (simple) or
\usepackage{soul} % use this (many fancier options)
\makeatother
\numberwithin{equation}{section}
\numberwithin{table}{section}
\allowdisplaybreaks

% -------------------------------------------------
% check references
% -------------------------------------------------
% \usepackage{refcheck}
% \usepackage[notref,notcite]{showkeys}
% \usepackage[notcite]{showkeys}
% \usepackage{showkeys}

% -------------------------------------------------
% cmark and xmark
% -------------------------------------------------

\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% -------------------------------------------------
% Environments here
% -------------------------------------------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{hypothesis}{Hypothesis}[section]
\newtheorem{assumption}{Assumption}[section]

\newtheorem{remark}{Remark}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{example}{Example}[section]

% -------------------------------------------------
%  Define short hand symbols.
% -------------------------------------------------
\newcommand{\E}{\mathbb{E}}
\newcommand{\W}{\dot{W}}
\newcommand{\ud}{\ensuremath{\mathrm{d} }}
\newcommand{\Ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\Floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\sgn}{\text{sgn}}
\newcommand{\Lad}{\text{L}_{\text{ad}}^2}
\newcommand{\SI}[1]{\mathcal{I}\left[#1 \right]}
\newcommand{\SIB}[2]{\mathcal{I}_{#2}\left[#1 \right]}
\newcommand{\Indt}[1]{1_{\left\{#1 \right\} }}
\newcommand{\LadInPrd}[1]{\left\langle #1 \right\rangle_{\text{L}_\text{ad}^2}}
\newcommand{\LadNorm}[1]{\left|\left|  #1 \right|\right|_{\text{L}_\text{ad}^2}}
\newcommand{\Norm}[1]{\left|\left|  #1   \right|\right|}
\newcommand*{\one}{{{\rm 1\mkern-1.5mu}\!{\rm I}}}
\newcommand{\Ito}{It\^{o} }
\newcommand{\Itos}{It\^{o}'s }
\newcommand{\spt}[1]{\text{supp}\left(#1\right)}
\newcommand{\InPrd}[1]{\left\langle #1 \right\rangle}
\newcommand{\mr}{\textbf{r}}
\newcommand{\Ei}{\text{Ei}}
\newcommand{\arctanh}{\operatorname{arctanh}}
\newcommand{\ind}[1]{\mathbb{I}_{\left\{ {#1} \right\} }}
\newcommand{\Pro}{\mathbb{P}}

\newcommand{\FoxH}[5]{H_{#2}^{#1}\left(#3\:\middle\vert\: \begin{subarray}{l}#4\\[0.4em] #5\end{subarray}\right)}

\DeclareMathOperator{\esssup}{\ensuremath{ess\,sup}}

\newcommand{\steps}[1]{\vskip 0.3cm \textbf{#1}}
\newcommand{\MFC}[1]{\href{https://mathscinet.ams.org/mathscinet/msc/msc2020.html?s=#1&btn=Current}{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\myEnd}{\hfill$\square$}
\newcommand{\ds}{\displaystyle}
\newcommand{\Shi}{\text{Shi}}
\newcommand{\Chi}{\text{Chi}}
\newcommand{\Daw}{\ensuremath{\mathrm{daw} }}
\newcommand{\Erf}{\ensuremath{\mathrm{erf} }}
\newcommand{\Erfi}{\ensuremath{\mathrm{erfi} }}
\newcommand{\Erfc}{\ensuremath{\mathrm{erfc} }}
\newcommand{\He}{\ensuremath{\mathrm{He} }}
\newcommand{\Var}{\ensuremath{\mathrm{Var} }}
\renewcommand{\Re}{\ensuremath{\mathrm{Re} }}
\newcommand{\Res}{\mathop{\text{Res}}}
\newcommand\calH{\mathcal{H}}
\newcommand{\argmin}{\ensuremath{\mathrm{Argmin}}}

\newcommand\crtL{\theta}

\newcommand{\conRef}[1]{(#1)}

\DeclareMathOperator{\Lip}{\mathit{L}}
\DeclareMathOperator{\LIP}{Lip}
\DeclareMathOperator{\lip}{\mathit{l}}

\DeclareMathOperator{\Vip}{\overline{\varsigma}}
\DeclareMathOperator{\vip}{\underline{\varsigma}}
\DeclareMathOperator{\vv}{\varsigma}
\DeclareMathOperator{\BC}{BC}
\DeclareMathOperator{\CH}{CD}
\DeclareMathOperator{\sd}{\beta}

\newcommand{\Dxa}{{}_x D_\delta^a}
\newcommand{\Dtb}{{}_t D_*^\beta}
\newcommand{\DRL}[2]{{}_t D_{#1}^{#2}}
\newcommand{\lMr}[3]{\:{}_{#1} #2_{#3}}
\newcommand{\tlMr}[4]{\:{}^{\hspace{0.2em}#1}_{#2} \hspace{-0.1em}#3_{#4}}

\newcommand{\myCmts}[1]{{\color{red}{\em !!} #1\hfill {\em !!}}\\}

\newcommand{\h}{\H}

% -------------------------------------------------
% BibTex setup
% -------------------------------------------------
\usepackage{amsrefs}

\renewcommand{\MR}[1]{~\href{https://mathscinet.ams.org/mathscinet-getitem?mr=MR#1}{MR#1}.}

\BibSpec{article}{%
+{}  {\PrintAuthors}                {author}
+{,} { \textit}                     {title}
+{.} { }                            {part}
+{:} { \textit}                     {subtitle}
+{,} { \PrintContributions}         {contribution}
+{.} { \PrintPartials}              {partial}
+{,} { }                            {journal}
+{}  { \textbf}                     {volume}
+{}  { \PrintDatePV}                {date}
+{,} { \issuetext}                  {number}
+{,} { \eprintpages}                {pages}
+{,} { }                            {status}
+{,} { \url}                        {url}
+{,} { \PrintDOI}                   {doi}
+{,} { available at \eprint}        {eprint}
+{}  { \parenthesize}               {language}
+{}  { \PrintTranslation}           {translation}
+{;} { \PrintReprint}               {reprint}
+{.} { }                            {note}
+{.} {}                             {transition}
+{}  {\SentenceSpace \PrintReviews} {review}
}

\BibSpec{book}{%
+{}  {\PrintAuthors}                {author}
+{,} { \textit}                     {title}
+{.} { }                            {part}
+{:} { \textit}                     {subtitle}
+{,} { \PrintEdition}               {edition}
+{,} { \PrintContributions}         {contribution}
+{,} { }                            {series}
+{,} { vol.~}                       {volume}
+{,} { }                            {publisher}
+{,} { }                            {organization}
+{,} { }                            {address}
+{,} { \PrintDateB}                 {date}
+{,} { }                            {status}
+{,} { \url}                        {url}
+{,} { \PrintDOI}                   {doi}
+{}  { \parenthesize}               {language}
+{}  { \PrintTranslation}           {translation}
+{;} { \PrintReprint}               {reprint}
+{.} { }                            {note}
+{.} {}                             {transition}
+{}  {\SentenceSpace \PrintReviews} {review}
}

\BibSpec{misc}{%
+{}  {\PrintAuthors}                {author}
+{,} { \textit}                     {title}
+{,} { }                            {publisher}
+{}  { \PrintDatePV}                {date}
+{,} { \url}                        {url}
+{,} { \PrintDOI}                   {doi}
+{.} { }                            {note}
+{.} {}                             {transition}
+{}  {\SentenceSpace \PrintReviews} {review}
}
% }}}


% \usepackage{refcheck}

